C-STS: Conditional Semantic Textual Similarity

Semantic textual similarity (STS), a cornerstone task in NLP, measures the degree of similarity between a pair of sentences, and has broad application in fields such as information retrieval and natural language understanding. However, sentence similarity can be inherently ambiguous, depending on the specific aspect of interest. We resolve this ambiguity by proposing a novel task called Conditional STS (C-STS) which measures sentences' similarity conditioned on an feature described in natural language (hereon, condition). As an example, the similarity between the sentences "The NBA player shoots a three-pointer." and "A man throws a tennis ball into the air to serve." is higher for the condition "The motion of the ball" (both upward) and lower for "The size of the ball" (one large and one small). C-STS's advantages are two-fold: (1) it reduces the subjectivity and ambiguity of STS and (2) enables fine-grained language model evaluation through diverse natural language conditions. We put several state-of-the-art models to the test, and even those performing well on STS (e.g. SimCSE, Flan-T5, and GPT-4) find C-STS challenging; all with Spearman correlation scores below 50. To encourage a more comprehensive evaluation of semantic similarity and natural language understanding, we make nearly 19K C-STS examples and code available for others to train and test their models.

==> LaTeX/300_background.tex <==
\section{Background}
\label{sec:background}

\hc{
\begin{enumerate}
    \item Cogsci motivated concepts of similarities
    \item Computer vision works on similarities \cite{veit_conditional_2017, parekh_crisscrossed_2021, ye_identifying_2022, parekh_crisscrossed_2021-1}
    \item NLP: STS related \cite{lopez-gazpio_interpretable_2017}
    \item NLP: conditioning related \cite{asai_task-aware_2022, su_one_2022}
    \item NLP: multi-view: \cite{he_multi-perspective_2015}
    \item NLP: NLI and data collection related \cite{nie_what_2020, abdalla_what_2021}
    \item learning disentangeld representations: IRM, invariant rationalization
    \item crowd sourcing: \cite{michael_crowdsourcing_2017}
\end{enumerate}
}

\paragraph{Historical perspectives of semantic similarities.}
Measuring similarities is a long standing problem spanning from cognitive science \cite{Miller1991Correlates}, psychology \cite{}, and linguistics \cite{}. \hc{what are their main approach to this problem and what are the major conclusions?}
In machine learning, similarity measurement focuses on \hc{mention CV etc}.

\paragraph{Textual similarity.}
Capturing textual similarity is also considered a fundamental problem in natural language processing. Works such as \citet{noauthor_semeval-2012_nodate, agirre_semeval-2016_2016, cer_semeval-2017_2017} defines the textual semantic similarity tasks (STS), which is widely used in common benchmarks such as GLUE \cite{wang2018glue}. 
Extensions to the STS setting has been proposed to identify the differences between the two sentences \cite{lopez-gazpio_interpretable_2017} as well as \hc{cite multi-lingua STS}. However, the issue of ambiguity as a core problem have not been made explicit.
Beyond STS, works that leverage conditioning to enhance sentence representations obtain improved performance for retrieval \cite{asai_task-aware_2022} and embedding qualities \cite{su_one_2022, he_multi-perspective_2015}, corroborating the observation that conditioning as a form of disambiguation benefits similarity measures.
In contrast to our work, \hc{blabla}

\paragraph{Crowdsourcing textual similarity pairs.}
